Toward Efficient Task Planning for Dual-Arm Tabletop Object Rearrangement

We investigate the problem of coordinating two robot arms to solve non-monotone tabletop multi-object rearrangement tasks. In a non-monotone rearrangement task, complex object-object dependencies exist that require moving some objects multiple times to solve an instance. In working with two arms in a large workspace, some objects must be handed off between the robots, which further complicates the planning process. For the challenging dual-arm tabletop rearrangement problem, we develop effective task planning algorithms for scheduling the pick-n-place sequence that can be properly distributed between the two arms. We show that, even without using a sophisticated motion planner, our method achieves significant time savings in comparison to greedy approaches and naive parallelization of single-robot plans.

==> 04-structural.tex <==
\begin{enumerate}
    \item In CMRF, computing RB or TB is equivalent to vertex separation problem and minimum removal problem
    \item Mention the hardness
    \item Introduce hardness on coordination
    \item two-arm system can increase efficiency to 3 times.
\end{enumerate}


==> 05-3-CMRF.tex <==
In CDRF, both robots can reach every corner of the workspace.
Handoff is not needed and all the pick-n-place manipulations can be executed by either arm.
This scenario is similar to the single arm rearrangement problem while the rearrangement plan can be executed by two arms.
This observation motivates us to first compute a task sequence as the single arm scenario and then split it into two subsequences of primitive actions with a task assigner.

The same as \cite{gao2021fast}, we choose DFDP for task sequences, which computes high-quality solutions efficiently.
When the makespan is measured in MC metric, the optimal task assignment is naive: $r_1$ executes tasks with odd indices and $r_2$ executes tasks with even indices.

When the makespan is measured in KC metric, the optimal task assignment can be found with a heuristic-guided search as well.
Given a node with depth $k$ in the search tree, it represents an task assignment on the first $k$ primitive actions and has two child nodes, indicating the assignment of the $(k+1)^{th}$ task to either $r_1$ or $r_2$.

Since the heuristic search is conducted based on a task ordering, 
we obey the ordering by requiring the starting moment of the release of the latter pick-n-place cannot be earlier than the finish moment of the grasp of the previous pick-n-place.
With this restriction, object-object collisions are avoided.

% \subsubsection{hold-n-place}
% Besides cooperation in task execution, the additional arm is able to reduce the number of temporary object displacements.
% Given a task sequence, an object $o_i$ is moved to the buffer at time $t_1$, and is moved out of the buffer at time $t_2$. 
% Alternatively, it can also be held by one arm at $t_1$ and be released at $t_2$.




==> 05-4-CMRN.tex <==
We also designed an algorithm for disjointed CDRN, which is CDRN with a further assumption that objects at start or goal positions in $\mathcal S(r_1)$ do not collide with the objects at start or goal positions in $\mathcal S(r_1)$.
This scenario mimics the situation where two arms rearrange objects on different workspaces(e.g. two different tables) and pass objects via handoff operations.
Motivated by the relatively isolated workspaces of two robots, 
we compute single arm rearrangement plans individually for both robots and then adjust the plan to coordinate the handoff moments.

For each arm $r_i$, the rearrangement in the workspace can be considered as a single arm rearrangement problem with three kinds of objects: (1) \emph{local objects} that do not need handoffs; (2) \emph{outgoing objects} that need handoffs to move away from $\mathcal S(r_1)$, (3) \emph{incoming objects} that need handoffs to move into $\mathcal S(r_1)$.
Fig.~\ref{fig:CDRN-Exp} shows a CDRN example with the instance on the left and the corresponding dependency graph on the right. For arm $r_1$, $o_5$, $o_6$, and $o_7$ are local objects, $o_1$ is the outgoing object, and $o_2$ is the incoming object.
For arm $r_2$, $o_3$ and $o_4$ are local objects, $o_2$ is the outgoing object, and $o_1$ is the incoming object.
In two disjointed regions, the corresponding dependency subgraphs are presented in Fig.~\ref{fig:CDRN-disjointed-graphs}. 
Each subgraph indicates the constraints in the corresponding region.
Based on the subgraphs, the primitive plans for two robot arms can be computed individually.
Fig.~\ref{fig:CDRN-coordinating-plans}[Left] shows a pair of resulting primitive plans. While the manipulations of local objects do not affect the rearrangement in the other half of the workspace, the handoff moments need further coordination.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/CMRN-Exp.jpg}
    \caption{An example of CDRN. [Left] start and goal positions in the workspace. [Right] The corresponding dependency graph. }
    \label{fig:CDRN-Exp}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/disjointed_graphs.png}
    \caption{Dependency subgraphs of Fig~\ref{fig:CDRN-Exp}[Right] of the disjointed regions. }
    \label{fig:CDRN-disjointed-graphs}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/coordinating_plans.png}
    \caption{[Left] A pair of primitive plans computed individually. [Right] The primitive plans after coordination. } 
    \label{fig:CDRN-coordinating-plans}
\end{figure}

We observe that the outgoing objects do not depend on local objects and the incoming objects are not depended by local objects.
Therefore, when the primitive plan suggests a moment for an outgoing handoff,
the moment can always be advanced. 
When the primitive plan suggests a moment for an incoming handoff, 
it can always be postponed.
In other words, a primitive plan provides right bounds for the outgoing handoffs and left bounds for the incoming handoffs on the timeline.

Based on the observation, we formulate an linear programming model to coordinate handoff moments. 
Denote $\mathcal O_h$ as the set of objects that need handoffs. 
For all $o_i\in \mathcal O_h$, let non-negative real variable $h_i$ represent the manipulation number of local objects before the handoff of $o_i$.
Constraints~\ref{eq:e1c1} indicate the safe bounds of the handoff timings. $t_{i1}$ and $t_{i2}$ are suggested by the computed primitive plans.
Constraints~\ref{eq:e1c2} indicate object dependencies. 
$E(\mathcal G)$ is the arc set of the dependency graph.
\begin{equation}\label{eq:e1c1}
    t_{i1}\leq h_i\leq t_{i2} \ \ \ o_i \in O_h
\end{equation}
\begin{equation}\label{eq:e1c2}
    h_i < h_j \ \ \ \forall (j,i)\in E(\mathcal G), o_i, o_j \in O_h
\end{equation}

In the working example Fig.~\ref{fig:CDRN-Exp}, the constraints for the handoffs are:
\begin{equation*}
    \begin{split}
        1\leq h_1\leq 3\\
        0\leq h_2\leq 1\\
        h_2 < h_1\\
    \end{split}
\end{equation*}

There is a feasible solution $h_1=2, h_2=1$. 
And the coordinated plans are presented in Fig.\ref{fig:CDRN-coordinating-plans}[Right].
In more difficult instances, not all handoff moments can be coordinated based on the primitive plans.
Therefore, we introduce Boolean variables $z_i$ to represent whether the handoffs obey all the constraints.
When there is no valid value for a handoff timing $h_i$,
it will be handoffed to a buffer location and moved to goal position at the end of the plan.
In other words, violation is allowed but might lead to additional cost in the makespan.
The constraints can be linearly represented as follows. 
The objective function maximizes the number of coordinated handoffs.
When $z_i=1$, constraints~\ref{eq:e2c1}-\ref{eq:e2c2} are equivalent to constraints~\ref{eq:e1c1}.
When $z_i=0$, constraints are satisfied but with penalty on the objective function.
Similarly, when $z_i=1$, constraints~\ref{eq:e2c3} are equivalent to constraints~\ref{eq:e1c2}.
When $z_i=0$, constraints are satisfied but with penalty on the objective function.
\begin{equation}\label{eq:e2o}
    argmax \sum_{o_i \in O_h} z_i \ \ \  \text{subject to}
\end{equation}
\begin{equation}\label{eq:e2c1}
    (h_i-t_{i1})+n(1-z_i)\geq 0 \ \ \  o_i \in O_h
\end{equation}
\begin{equation}\label{eq:e2c2}
    (t_{i2}-h_i)+n(1-z_i)\geq 0 \ \ \  o_i \in O_h
\end{equation}
\begin{equation}\label{eq:e2c3}
\begin{split}
    (h_i - h_j)+n(1-z_i)+n(1-z_j) \geq 1/n \\ 
    \forall (i,j)\in E(\mathcal G), o_i, o_j \in O_h
\end{split}
\end{equation}


% As for the dependencies, there is no arc between local objects of $r_1$ and those of $r_2$, due to the assumption of disjointed CDRF.
% Also, local objects may have dependencies on out-going objects, e.g. $o_6$ depends on $o_3$. 
% Moreover, in-coming objects may have dependencies on both local objects and out-going objects.
% Intuitively speaking, a ``selfishless'' robot arm will request for in-coming handoffs as soon as possible and withhold the out-going handoffs until the end of the rearrangement in order to reduce task difficulty of the other arm.


